Semantics-Guided Synthesis

This paper develops a new framework for program synthesis, called semantics-guided synthesis (SemGuS), that allows a user to provide both the syntax and the semantics for the constructs in the language. SemGuS accepts a recursively defined big-step semantics, which allows it, for example, to be used to specify and solve synthesis problems over an imperative programming language that may contain loops with unbounded behavior. The customizable nature of SemGuS also allows synthesis problems to be defined over a non-standard semantics, such as an abstract semantics. In addition to the SemGuS framework, we develop an algorithm for solving SemGuS problems that is capable of both synthesizing programs and proving unrealizability, by encoding a SemGuS problem as a proof search over Constrained Horn Clauses: in particular, our approach is the first that we are aware of that can prove unrealizabilty for synthesis problems that involve imperative programs with unbounded loops, over an infinite syntactic search space. We implemented the technique in a tool called MESSY, and applied it to both SyGuS problems(i.e., over expressions) and synthesis problems over an imperative programming language.

==> additional-eval.tex <==
\section{Additional Evaluation}
\label{Se:AdditionalEval}

\input{resulttable}

==> fused-semantics.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Inference Rules for the Fused Semantics}
\label{Se:InferenceRulesForTheFusedSemantics}

$
\infer[\textit{fuse}^\rsZero_{E \rightarrow 0 \sball{j}}]
{\fEFrreduce{\VG, \aI}{\Vv, j::\aI}}
{
  Zero^v(\VG) = \Vv
} \qquad
\infer[\textit{fuse}^\rsOne_{E \rightarrow 1 \sball{j}}]{\fEFrreduce{\VG, \aI}{\Vv, j::\aI}}
{
  One^v(\VG) = \Vv
}
$\\

$
\infer[\textit{fuse}^{\mathsf{Var_s}}_{E \rightarrow x \sball{j}}]{\fEFrreduce{\VG, \aI}{\Vect{v}, j::\aI}}
  {
    Var^v(\VG, \Vect{x}) = \Vect{v}
  }
$\\

$
\infer[\textit{fuse}^\rsAdd_{E \rightarrow E_1+E_2 \sball{j}}]{\fEFrreduce{\VG, \aI}{\Vv, j::\aI_2}}
{
  \fEFnrreduce{1}{\VG, \aI_1}{\Vv_1, \aI_2} \quad
  \fEFnrreduce{2}{\VG, \aI}{\Vv_2, \aI_1} \quad
  +^v(\VG, \Vv_1, \Vv_2) = \Vv
}
$\\

$
\infer[
\textit{fuse}^\rsEITE_{E \rightarrow \Eifthenelse{B}{E_1}{E_2} \sball{j}}
]
{\fEFrreduce{\VG, \aI}{\Vv, \aI_3}}
{
\begin{array}{c}
\fBFrreduce{\VG, \aI_2}{\Vv_b, \aI_3} \quad
  \fEFnrreduce{1}{\Vproj{\VG}{\Vv_b}, \aI_1}{\Vv_1, \aI_2}\\
  \fEFnrreduce{2}{\Vproj{\VG}{\lnot \Vv_b}, \aI}{\Vv_2, \aI_1} \qquad 
  EITE^v(\VG, \Vv_b, \Vv_1, \Vv_2) = \Vv
\end{array}  
}
$\\

$
\infer[\textit{fuse}^\rsTrue_{B \rightarrow \Etrue \sball{j}}]{\fBFrreduce{\VG, \aI}{\Vv, j::\aI}}
{
  True^v(\VG) = \Vv
} \qquad
\infer[\textit{fuse}^\rsFalse_{B \rightarrow \Efalse \sball{j}}]{\fBFrreduce{\VG, \aI}{\Vv, j::\aI}}
{
  False^v(\VG) = \Vv
}
$\\

$
\infer[\textit{fuse}^\rsNot_{B \rightarrow \lnot B_1 \sball{j}}]{\fBFrreduce{\VG, \aI}{\Vv, j::\aI_1}}
{
  \fBFnrreduce{1}{\VG, \aI}{\Vv_b, \aI_1} \quad
  \lnot^v(\VG, \Vv_b) = \Vv
}
$\\

$
\infer[\textit{fuse}^\rsAnd_{B \rightarrow B_1\wedge B_2 \sball{j}}]{\fBFrreduce{\VG, \aI}{\Vv, j::\aI_2}}
{
  \fBFnrreduce{1}{\VG, \aI_1}{\Vv_1, \aI_2} \quad
  \fBFnrreduce{2}{\VG, \aI}{\Vv_2, \aI_1} \quad
  \wedge^v(\VG, \Vv_1, \Vv_2) = \Vv
}
$\\


$
\infer[\textit{fuse}^{\rsComp}_{B \rightarrow E_1 < E_2 \sball{j}}]{\fBFrreduce{\VG, \aI}{\Vv, j::\aI_2}}
{
\fEFnrreduce{1}{\VG, \aI_1}{\Vv_1, \aI_2} \quad
  \fEFnrreduce{2}{\VG, \aI}{\Vv_2, \aI_1} \quad
  <^v(\VG, \Vv_1, \Vv_2) = \Vv
}
$\\

$
\infer[\textit{fuse}^\mathsf{Assign_s}_{S \rightarrow x := E \sball{j}}]{\fSFrreduce{\VG, \aI}{\VG_r, j::\aI_1}}
  {
    \fEFrreduce{\VG, \aI}{\Vect{e}, \aI_1} \quad
    Update^{v}(\VG, \Vect{x}, \Vect{e}) = \VG_r
  }
$\\


$
\infer[\textit{fuse}^\rsSeq_{S \rightarrow S_1 ; S_2 \sball{j}}]{\fSFrreduce{\VG, \aI}{\VG_r, j::\aI_2}}
{
    \fSFnrreduce{1}{\VG, \aI_1}{\VG_1, \aI_2} \quad
    \fSFnrreduce{2}{\VG_1, \aI}{\VG_2, \aI_1} \quad
  Seq^v(\VG, \VG_1, \VG_2) = \VG_r
}
$\\



$
\infer[\textit{fuse}^\rsSITE_{S \rightarrow \Eifthenelse{B}{S_1}{S_2} \sball{j}}]
{\fSFrreduce{\VG, \aI}{\VG_r, j::\aI_3}}
{
\begin{array}{c}
  \fBFrreduce{\VG, \aI_2}{\Vv_b, \aI_3} \quad
  \fSFnrreduce{1}{\Vproj{\VG}{\Vv_b}, \aI_1}{\VG_1, \aI_2}\\
  \fSFnrreduce{2}{\Vproj{\VG}{\lnot \Vv_b}, \aI}{\VG_2, \aI_1} \quad
  SITE^v(\VG, \Vv_b, \VG_1, \VG_2) = \VG_r
\end{array}  
}
$\\

$
\infer[\textit{fuse}^\rsWT_{S \rightarrow \Ewhile{B}{S_1} \sball{j}}]{\fSFrreduce{\VG, \aI}{\VG_r, j::\aI_2}}
{
\begin{array}{c}
\fBFrreduce{\VG, \aI_1}{\Vv_b, \aI_2} \quad
\Etrue \in \Vv_b \quad
  \fSFnrreduce{1}{\Vproj{\VG}{\Vv_b}, \aI}{\VG_1, \aI_1} \\
  \SFlreduce{\VG_1, j::\aI_2}{\VG_2, \aI_3} \quad
  WTrue^v(\VG, \Vv_b, \VG_1, \VG_2) = \VG_r 
\end{array}  
}
$\\

$
\infer[\textit{sem}^\rsZero_{E \rightarrow 0 \sball{j}}]{\EFlreduce{\VG, j::\aI}{\Vv, \aI}}
{
  Zero^v(\VG) = \Vv
} \qquad
\infer[\textit{sem}^\rsOne_{E \rightarrow 1 \sball{j}}]{\EFlreduce{\VG, j::\aI}{\Vv, \aI}}
{
  One^v(\VG) = \Vv
}
$\\

$
\infer[\textit{sem}^{\mathsf{Var_s}}_{E \rightarrow x \sball{j}}]{\EFlreduce{\VG, j::\aI}{\Vect{v}, \aI}}
  {
    Var^v(\VG, \Vect{x}) = \Vect{v}
  }
$\\

$
\infer[ \textit{sem}^\rsAdd_{E \rightarrow E_1 + E_2 \sball{j}}]{\EFlreduce{\VG, j::\aI}{\Vv, \aI_2}}
{
  \EFnlreduce{1}{\VG, \aI}{\Vv_1, \aI_1} \quad
  \EFnlreduce{2}{\VG, \aI_1}{\Vv_2, \aI_2} \quad
  +^v(\VG, \Vv_1, \Vv_2) = \Vv
}
$\\\\\\



$
\infer[\textit{sem}^\rsEITE_{E \rightarrow \Eifthenelse{B}{E_1}{E_2} \sball{j}}]{\EFlreduce{\VG, j::\aI}{\Vv, \aI_3}}
{
\begin{array}{c}
\BFlreduce{\VG, \aI}{\Vv_b, \aI_1} \quad
  \EFnlreduce{1}{\Vproj{\VG}{\Vv_b}, \aI_1}{\Vv_1, \aI_2}\\
  \EFnlreduce{2}{\Vproj{\VG}{\lnot \Vv_b}, \aI_2}{\Vv_2, \aI_3} \quad 
  EITE^v(\VG, \Vv_b, \Vv_1, \Vv_2) = \Vv
  \end{array}
}
$\\

$
\infer[\textit{sem}^\rsTrue_{B \rightarrow \Etrue \sball{j}}]{\BFlreduce{\VG, j::\aI}{\Vv, \aI}}
{
  True^v(\VG) = \Vv
} \qquad
\infer[\textit{sem}^\rsFalse_{B \rightarrow \Efalse \sball{j}}]{\BFlreduce{\VG, j::\aI}{\Vv, \aI}}
{
  False^v(\VG) = \Vv
}
$\\

$
\infer[\textit{sem}^\rsNot_{B \rightarrow \lnot B_1 \sball{j}}]{\BFlreduce{\VG, j::\aI}{\Vv, \aI_1}}
{
  \BFnlreduce{1}{\VG, \aI}{\Vv_b, \aI_1} \quad
  \lnot^v(\VG, \Vv_b) = \Vv
}
$\\

$
\infer[\textit{sem}^\rsAnd_{B \rightarrow B_1 \wedge B_2 \sball{j}}]{\BFlreduce{\VG, j::\aI}{\Vv, \aI_2}}
{
  \BFnlreduce{1}{\VG, \aI}{\Vv_1, \aI_1} \quad
  \BFnlreduce{2}{\VG, \aI_1}{\Vv_2, \aI_2} \quad
  \wedge^v(\VG, \Vv_1, \Vv_2) = \Vv
}
$\\


$
\infer[\textit{sem}^{\rsComp}_{B \rightarrow E_1 < E_2 \sball{j}}]{\BFlreduce{\VG, j::\aI}{\Vv, \aI_2}}
{
  \EFnlreduce{1}{\VG, \aI}{\Vv_1, \aI_1} \quad
  \EFnlreduce{2}{\VG, \aI_1}{\Vv_2, \aI_2} \quad
  <^v(\VG, \Vv_1, \Vv_2) = \Vv
}
$\\

$
\infer[\textit{sem}^\mathsf{Assign_s}_{S \rightarrow x := E \sball{j}}]{\SFlreduce{\VG, j::\aI}{\VG_r, \aI_1}}
  {
    \EFlreduce{\VG, \aI}{\Vect{e}, \aI_1} \quad
    Update^{v}(\VG, \Vect{x}, \Vect{e}) = \VG_r
  }
$\\


$
\infer[\textit{sem}^\rsSeq_{S \rightarrow S_1;S_2 \sball{j}}]{\SFlreduce{\VG, j::\aI}{\VG_r, \aI_2}}
{
  \SFnlreduce{1}{\VG, \aI}{\VG_1, \aI_1} \quad
  \SFnlreduce{2}{\VG_1, \aI_1}{\VG_2, \aI_2} \quad
  Seq^v(\VG, \VG_1, \VG_2) = \VG_r
}
$\\


$
\infer[\textit{sem}^\rsSITE_{S \rightarrow \Eifthenelse{B}{S_1}{S_2} \sball{j}}]{\SFlreduce{\VG, j::\aI}{\VG_r, \aI_3}}
{
\begin{array}{c}
\BFlreduce{\VG, \aI}{\Vv_b, \aI_1} \quad
  \SFnlreduce{1}{\Vproj{\VG}{\Vv_b}, \aI_1}{\VG_1, \aI_2}\\
  \SFnlreduce{2}{\Vproj{\VG}{\lnot \Vv_b}, \aI_2}{\VG_2, \aI_3} \quad
  SITE^v(\VG, \Vv_b, \VG_1, \VG_2) = \VG_r
\end{array}  
}
$\\


$
\infer[\textit{sem}^\rsWT_{S \rightarrow \Ewhile{B}{S_1} \sball{j}}]{\SFlreduce{\VG, j::\aI}{\VG_r, \aI_3}}
{
\begin{array}{c}
\BFlreduce{\VG, \aI}{\Vv_b, \aI_1} \quad
\Etrue \in \Vv_b\\
  \SFnlreduce{1}{\Vproj{\VG}{\Vv_b}, \aI_1}{\VG_1, \aI_2} \quad
  \SFlreduce{\VG_1, j::\aI}{\VG_2, \aI_3} \\
  WTrue^v(\VG, \Vv_b, \VG_1, \VG_2) = \VG_r 
\end{array}  
}
$\\


$
\infer[\textit{sem}^\rsWF_{S \rightarrow \Ewhile{B}{S_1} \sball{j}}]{\SFlreduce{\VG, j::\aI}{\VG_r, \aI_2}}
{
\begin{array}{c}
\BFlreduce{\VG, \aI}{\Vv_b, \aI_1} \quad
\Etrue \not \in \Vv_b\\
  \SFnlreduce{1}{\Vproj{\VG}{\Vv_b}, \aI_1}{\VG_1, \aI_2} \quad
  WFalse^v(\VG, \Vv_b, \VG_1) = \VG_r
\end{array}  
}
$

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper.tex"
%%% End: 


==> resulttable2.tex <==
	\begin{table}
	\caption{
		Performance of \name and \namenay  for \textsc{LimitedIf} and \textsc{LimitedPlus} benchmarks over examples produced by CEGIS-random.
		The table shows the number of nonterminals ($|N|$), productions ($|\delta|$), and variables ($|V|$)
		in the problem grammar; the number of examples produced in the CEGIS loop ($|E|$);
		and the running time of \name and \namenay.		\xmark\ denotes a timeout.}
		\footnotesize
		\centering
		\begin{tabular}{cc|rrr|rr|rr}
		&	 \multirow{2}{*}{\bf Problem} & \multicolumn{3}{c|}{\bf Grammar}& \multirow{2}{*}{\bf $|E|$} &  {\bf \name}  & {\bf \namenay} \\
			 &  &  {\bf $|N|$}  &  {\bf $|\delta|$} & {\bf $|V|$} & &\multirow{1}{*}{\bf time (s)} & \multirow{1}{*}{\bf $|E|$} &\multirow{1}{*}{\bf time (s)}  \\
			    \hline
\parbox[t]{-11mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{\textsc{LimitedPlus}}}}														
& guard1	&	7	&	24	&	3	&	2	&	0.41	&	&	0.2	\\
& guard2	&	9	&	34	&	3	&	3	&	21.51	&	&	1.12	\\
& guard3	&	11	&	41	&	3	&	1	&	0.07	&	&	2.88	\\
& guard4*	&	11	&	72	&	3	&	3.5	&	72.58	&	&	1.93	\\
& plane1	&	2	&	5	&	2	&	1	&	0.12	&	&	0.02	\\	
& plane2	&	17	&	60	&	2	&	1.6	&	1.24	&	&	7.51	\\	
& plane3	&	29	&	122	&	2	&	1.5	&	25.42	&	&	95.17	\\	
& ite1*	&	7	&	2	&	3	&	2	&	2.07	&	&	0.13	\\	
& ite2*	&	9	&	34	&	3	&	4	&	29.54	&	&	45.67	\\	
&  sum\_2\_5	&	11	&	40	&	2	&	4	&	20.47	&	&	15.65	\\
&  search\_2	&	5	&	16	&	3	&	3	&	2	&	&	0.13	\\	
&  search\_3	&	7	&	25	&	4	&	4	&	4.81	&	&	0.36	\\	
\hdashline														
\parbox[t]{1mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{\textsc{LimitedIf}}}}														
&max2	&	1	&	5	&	2	&	4	&	0.18	&	&	1.48	\\	
&max3	&	3	&	15	&	3	&	9	&	9.67	&	&	\xmark	\\	
&  sum\_2\_5	&	1	&	5	&	2	&	3	&	0.26	&	&	0.69	\\	
&  sum\_2\_15	&	1	&	5	&	2	&	3	&	0.26	&	&	0.87	\\	
&  sum\_3\_5	&	3	&	15	&	3	&	8	&	29.85	&	&	\xmark	\\	
&  sum\_3\_15	&	3	&	15	&	3	&	9	&	31.03	&	&	\xmark	\\	
&  search\_2	&	3	&	15	&	3	&	5	&	29.92	&	&	\xmark	\\	
& example1	&	3	&	10	&	2	&	3	&	0.16	&	&	6.54	\\	
& guard1	&	1	&	6	&	2	&	4	&	0.14	&	&	0.46	\\	
& guard2	&	1	&	6	&	2	&	4	&	0.24	&	&	0.23	\\	
& guard3	&	1	&	6	&	2	&	4	&	0.25	&	&	0.85	\\	
& guard4	&	1	&	6	&	2	&	4	&	0.13	&	&	0.21	\\	
& ite1	&	3	&	15	&	3	&	-	&	5.35	&	&	\xmark	\\	
%			 ite1 &	8  & 32 & 3 & - & - & - & - & - & \xmark & \xmark & \xmark &  \xmark &  \xmark\\
%			 ite2 & 10 & 42 & 3 & - & - & - & - & - & \xmark & \xmark & \xmark &  \xmark &  \xmark\\
			
%			 guard4 & 14 & 60 & 3 &  - & - & - & - & - & \xmark & \xmark & \xmark &  \xmark &  \xmark\\
%			 example1 & 52 & 336 & 2 &- & - & - & - & - & \xmark & \xmark & \xmark &  \xmark &  \xmark\\
%			  sum\_2\_5 & 12 & 47 & 2 &- & - & - & - & - & \xmark & \xmark & \xmark &  \xmark &  \xmark\\

\end{tabular}
\label{Ta:results2}
\end{table}
